Deep Learning Techniques for Improving Digital Gait Segmentation

Wearable technology for the automatic detection of gait events has recently gained growing interest, enabling advanced analyses that were previously limited to specialist centres and equipment (e.g., instrumented walkway). In this study, we present a novel method based on dilated convolutions for an accurate detection of gait events (initial and final foot contacts) from wearable inertial sensors. A rich dataset has been used to validate the method, featuring 71 people with Parkinson's disease (PD) and 67 healthy control subjects. Multiple sensors have been considered, one located on the fifth lumbar vertebrae and two on the ankles. The aims of this study were: (i) to apply deep learning (DL) techniques on wearable sensor data for gait segmentation and quantification in older adults and in people with PD; (ii) to validate the proposed technique for measuring gait against traditional gold standard laboratory reference and a widely used algorithm based on wavelet transforms (WT); (iii) to assess the performance of DL methods in assessing high-level gait characteristics, with focus on stride, stance and swing related features. The results showed a high reliability of the proposed approach, which achieves temporal errors considerably smaller than WT, in particular for the detection of final contacts, with an inter-quartile range below 70 ms in the worst case. This study showes encouraging results, and paves the road for further research, addressing the effectiveness and the generalization of data-driven learning systems for accurate event detection in challenging conditions.

==> result_table.tex <==
\begin{tabular}{lrrr}
\toprule
{} &  Event Network &  Khandelwal &  McCamley \\
\midrule
IC (CT) - bias                   &          0.000 &       0.047 &     0.086 \\
IC (CT) - IQR                    &          0.047 &       0.062 &     0.164 \\
IC (PD) - bias                   &         -0.008 &       0.023 &     0.094 \\
IC (PD) - IQR                    &          0.062 &       0.078 &     0.117 \\
FC (CT) - bias                   &          0.000 &      -0.070 &     0.055 \\
FC (CT) - IQR                    &          0.039 &       0.070 &     0.531 \\
FC (PD) - bias                   &         -0.008 &      -0.102 &     0.039 \\
FC (PD) - IQR                    &          0.070 &       0.086 &     0.477 \\
IC (CT) - Precision              &          0.910 &       0.900 &     0.261 \\
IC (CT) - Recall                 &          0.864 &       0.836 &     0.206 \\
IC (PD) - Precision              &          0.890 &       0.802 &     0.258 \\
IC (PD) - Recall                 &          0.835 &       0.752 &     0.209 \\
FC (CT) - Precision              &          0.916 &       0.570 &     0.283 \\
FC (CT) - Recall                 &          0.858 &       0.436 &     0.216 \\
FC (PD) - Precision              &          0.859 &       0.305 &     0.423 \\
FC (PD) - Recall                 &          0.800 &       0.226 &     0.328 \\
Stride Average (CT\_2) - bias     &          0.000 &       0.000 &     0.000 \\
Stride Average (CT\_2) - IQR      &          0.006 &       0.008 &     0.008 \\
Stride Average (CT\_3) - bias     &          0.000 &       0.000 &     0.000 \\
Stride Average (CT\_3) - IQR      &          0.004 &       0.004 &     0.004 \\
Stride Average (PD\_2) - bias     &          0.000 &       0.000 &     0.000 \\
Stride Average (PD\_2) - IQR      &          0.012 &       0.016 &     0.008 \\
Stride Average (PD\_3) - bias     &          0.000 &       0.000 &     0.000 \\
Stride Average (PD\_3) - IQR      &          0.008 &       0.014 &     0.008 \\
Stride Variability (CT\_2) - bias &         -0.006 &      -0.002 &    -0.004 \\
Stride Variability (CT\_2) - IQR  &          0.016 &       0.010 &     0.011 \\
Stride Variability (CT\_3) - bias &         -0.004 &       0.000 &    -0.004 \\
Stride Variability (CT\_3) - IQR  &          0.012 &       0.014 &     0.019 \\
Stride Variability (PD\_2) - bias &         -0.004 &      -0.008 &    -0.002 \\
Stride Variability (PD\_2) - IQR  &          0.020 &       0.334 &     0.016 \\
Stride Variability (PD\_3) - bias &         -0.002 &      -0.006 &    -0.004 \\
Stride Variability (PD\_3) - IQR  &          0.012 &       0.353 &     0.020 \\
Stride Asymmetry (CT\_2) - bias   &          0.000 &      -0.004 &     0.000 \\
Stride Asymmetry (CT\_2) - IQR    &          0.008 &       0.012 &     0.010 \\
Stride Asymmetry (CT\_3) - bias   &          0.000 &       0.000 &     0.000 \\
Stride Asymmetry (CT\_3) - IQR    &          0.012 &       0.008 &     0.010 \\
Stride Asymmetry (PD\_2) - bias   &         -0.004 &      -0.004 &     0.000 \\
Stride Asymmetry (PD\_2) - IQR    &          0.008 &       0.097 &     0.012 \\
Stride Asymmetry (PD\_3) - bias   &          0.000 &      -0.008 &     0.000 \\
Stride Asymmetry (PD\_3) - IQR    &          0.008 &       0.035 &     0.008 \\
Stance Average (CT\_2) - bias     &         -0.008 &       0.109 &     0.008 \\
Stance Average (CT\_2) - IQR      &          0.016 &       0.023 &     0.023 \\
Stance Average (CT\_3) - bias     &         -0.004 &       0.109 &     0.008 \\
Stance Average (CT\_3) - IQR      &          0.023 &       0.023 &     0.029 \\
Stance Average (PD\_2) - bias     &          0.000 &       0.125 &     0.016 \\
Stance Average (PD\_2) - IQR      &          0.016 &       0.040 &     0.039 \\
Stance Average (PD\_3) - bias     &          0.000 &       0.125 &     0.020 \\
Stance Average (PD\_3) - IQR      &          0.029 &       0.044 &     0.049 \\
Stance Variability (CT\_2) - bias &         -0.016 &       0.002 &    -0.004 \\
Stance Variability (CT\_2) - IQR  &          0.033 &       0.008 &     0.020 \\
Stance Variability (CT\_3) - bias &         -0.008 &       0.004 &    -0.006 \\
Stance Variability (CT\_3) - IQR  &          0.027 &       0.008 &     0.018 \\
Stance Variability (PD\_2) - bias &         -0.008 &       0.000 &     0.000 \\
Stance Variability (PD\_2) - IQR  &          0.027 &       0.036 &     0.023 \\
Stance Variability (PD\_3) - bias &         -0.008 &       0.000 &    -0.006 \\
Stance Variability (PD\_3) - IQR  &          0.017 &       0.023 &     0.018 \\
Stance Asymmetry (CT\_2) - bias   &         -0.012 &       0.000 &    -0.008 \\
Stance Asymmetry (CT\_2) - IQR    &          0.033 &       0.016 &     0.016 \\
Stance Asymmetry (CT\_3) - bias   &         -0.008 &       0.000 &    -0.004 \\
Stance Asymmetry (CT\_3) - IQR    &          0.023 &       0.012 &     0.016 \\
Stance Asymmetry (PD\_2) - bias   &         -0.008 &       0.000 &     0.000 \\
Stance Asymmetry (PD\_2) - IQR    &          0.027 &       0.020 &     0.027 \\
Stance Asymmetry (PD\_3) - bias   &         -0.008 &       0.002 &    -0.008 \\
Stance Asymmetry (PD\_3) - IQR    &          0.035 &       0.012 &     0.025 \\
Swing Average (CT\_2) - bias      &          0.000 &      -0.109 &    -0.004 \\
Swing Average (CT\_2) - IQR       &          0.023 &       0.023 &     0.023 \\
Swing Average (CT\_3) - bias      &          0.000 &      -0.109 &    -0.008 \\
Swing Average (CT\_3) - IQR       &          0.020 &       0.031 &     0.027 \\
Swing Average (PD\_2) - bias      &          0.000 &      -0.119 &    -0.020 \\
Swing Average (PD\_2) - IQR       &          0.020 &       0.039 &     0.043 \\
Swing Average (PD\_3) - bias      &          0.000 &      -0.125 &    -0.023 \\
Swing Average (PD\_3) - IQR       &          0.027 &       0.039 &     0.045 \\
Swing Variability (CT\_2) - bias  &         -0.010 &       0.000 &     0.000 \\
Swing Variability (CT\_2) - IQR   &          0.039 &       0.015 &     0.013 \\
Swing Variability (CT\_3) - bias  &         -0.008 &       0.000 &     0.000 \\
Swing Variability (CT\_3) - IQR   &          0.017 &       0.014 &     0.016 \\
Swing Variability (PD\_2) - bias  &         -0.008 &      -0.002 &     0.000 \\
Swing Variability (PD\_2) - IQR   &          0.025 &       0.019 &     0.023 \\
Swing Variability (PD\_3) - bias  &         -0.010 &       0.000 &    -0.002 \\
Swing Variability (PD\_3) - IQR   &          0.021 &       0.023 &     0.013 \\
Swing Asymmetry (CT\_2) - bias    &         -0.008 &       0.000 &    -0.004 \\
Swing Asymmetry (CT\_2) - IQR     &          0.031 &       0.012 &     0.020 \\
Swing Asymmetry (CT\_3) - bias    &         -0.004 &       0.000 &    -0.004 \\
Swing Asymmetry (CT\_3) - IQR     &          0.020 &       0.012 &     0.014 \\
Swing Asymmetry (PD\_2) - bias    &         -0.008 &       0.000 &     0.000 \\
Swing Asymmetry (PD\_2) - IQR     &          0.027 &       0.023 &     0.031 \\
Swing Asymmetry (PD\_3) - bias    &         -0.008 &       0.000 &    -0.004 \\
Swing Asymmetry (PD\_3) - IQR     &          0.031 &       0.019 &     0.021 \\
\bottomrule
\end{tabular}


==> result_table_prec_rec.tex <==
\begin{tabular}{llllllll}
\toprule
{} & {} & {} & Event Network & Event Network (ANK only) & Event Network (WT only) & Khandelwal & McCamley \\
\midrule
IC & CT & Precision &  \textbf{0.91} &                     0.89 &                    0.90 &       0.90 &     0.26 \\
IC & CT & Recall    &  \textbf{0.86} &                     0.84 &                    0.85 &       0.84 &     0.21 \\
IC & PD & Precision &  \textbf{0.89} &                     0.88 &                    0.85 &       0.80 &     0.26 \\
IC & PD & Recall    &  \textbf{0.84} &                     0.82 &                    0.79 &       0.75 &     0.21 \\
FC & CT & Precision &  \textbf{0.92} &                     0.90 &                    0.89 &       0.57 &     0.28 \\
FC & CT & Recall    &  \textbf{0.86} &                     0.84 &                    0.83 &       0.44 &     0.22 \\
FC & PD & Precision &          0.86 &             \textbf{0.86} &            \textbf{0.87} &       0.30 &     0.42 \\
FC & PD & Recall    &  \textbf{0.80} &                     0.79 &            \textbf{0.80} &       0.23 &     0.33 \\
\bottomrule
\end{tabular}


==> result_table_time_errors.tex <==
\begin{tabular}{lllllllll}
\toprule
{} & {} & {} & {} &   Event Network & Event Network (ANK only) & Event Network (WT only) &     Khandelwal &       McCamley \\
\midrule
Event & IC & CT & bias   &   \textbf{0.000} &                   -0.008 &           \textbf{0.000} &          0.047 &          0.086 \\
Event & IC & CT & IQR    &   \textbf{0.047} &                    0.055 &           \textbf{0.047} &          0.062 &          0.164 \\
Event & IC & PD & bias   &  \textbf{-0.008} &                   -0.016 &                  -0.016 &          0.023 &          0.094 \\
Event & IC & PD & IQR    &   \textbf{0.062} &                    0.070 &           \textbf{0.062} &          0.078 &          0.117 \\
Event & FC & CT & bias   &   \textbf{0.000} &                   -0.008 &           \textbf{0.000} &         -0.070 &          0.055 \\
Event & FC & CT & IQR    &   \textbf{0.039} &                    0.047 &                   0.055 &          0.070 &          0.531 \\
Event & FC & PD & bias   &  \textbf{-0.008} &                   -0.016 &                  -0.016 &         -0.102 &          0.039 \\
Event & FC & PD & IQR    &           0.070 &            \textbf{0.062} &           \textbf{0.062} &          0.086 &          0.477 \\
Avg & Stride & CT & bias &   \textbf{0.000} &            \textbf{0.000} &           \textbf{0.000} &  \textbf{0.000} &  \textbf{0.000} \\
Avg & Stride & CT & IQR  &           0.004 &            \textbf{0.000} &                   0.004 &          0.004 &          0.008 \\
Avg & Stride & PD & bias &   \textbf{0.000} &            \textbf{0.000} &           \textbf{0.000} &  \textbf{0.000} &  \textbf{0.000} \\
Avg & Stride & PD & IQR  &           0.008 &            \textbf{0.004} &           \textbf{0.004} &          0.012 &          0.008 \\
Avg & Stance & CT & bias &          -0.008 &            \textbf{0.000} &           \textbf{0.000} &          0.109 &          0.008 \\
Avg & Stance & CT & IQR  &           0.020 &            \textbf{0.016} &                   0.020 &          0.023 &          0.031 \\
Avg & Stance & PD & bias &   \textbf{0.000} &            \textbf{0.000} &           \textbf{0.000} &          0.125 &          0.016 \\
Avg & Stance & PD & IQR  &           0.023 &            \textbf{0.016} &                   0.031 &          0.042 &          0.047 \\
Avg & Swing & CT & bias  &   \textbf{0.000} &            \textbf{0.000} &           \textbf{0.000} &         -0.109 &         -0.008 \\
Avg & Swing & CT & IQR   &           0.020 &            \textbf{0.016} &           \textbf{0.016} &          0.023 &          0.027 \\
Avg & Swing & PD & bias  &   \textbf{0.000} &            \textbf{0.000} &           \textbf{0.000} &         -0.125 &         -0.021 \\
Avg & Swing & PD & IQR   &           0.020 &            \textbf{0.017} &                   0.031 &          0.039 &          0.044 \\
Var & Stride & CT & bias &          -0.005 &            \textbf{0.000} &                  -0.004 &  \textbf{0.000} &         -0.004 \\
Var & Stride & CT & IQR  &           0.014 &            \textbf{0.010} &                   0.012 &          0.012 &          0.016 \\
Var & Stride & PD & bias &          -0.003 &            \textbf{0.000} &           \textbf{0.000} &         -0.007 &         -0.002 \\
Var & Stride & PD & IQR  &           0.016 &            \textbf{0.014} &                   0.016 &          0.352 &          0.016 \\
Var & Stance & CT & bias &          -0.012 &            \textbf{0.000} &                  -0.008 &          0.002 &         -0.006 \\
Var & Stance & CT & IQR  &           0.029 &                    0.015 &                   0.023 &  \textbf{0.008} &          0.018 \\
Var & Stance & PD & bias &          -0.008 &                   -0.004 &                  -0.010 &  \textbf{0.000} &         -0.004 \\
Var & Stance & PD & IQR  &           0.023 &            \textbf{0.018} &                   0.029 &          0.030 &          0.020 \\
Var & Swing & CT & bias  &          -0.008 &                   -0.002 &                  -0.008 &  \textbf{0.000} &  \textbf{0.000} \\
Var & Swing & CT & IQR   &           0.027 &                    0.018 &                   0.025 &  \textbf{0.014} &  \textbf{0.014} \\
Var & Swing & PD & bias  &          -0.010 &                   -0.001 &                  -0.012 &  \textbf{0.000} &         -0.002 \\
Var & Swing & PD & IQR   &           0.023 &            \textbf{0.020} &                   0.023 &          0.023 &  \textbf{0.020} \\
Asy & Stride & CT & bias &   \textbf{0.000} &            \textbf{0.000} &           \textbf{0.000} &  \textbf{0.000} &  \textbf{0.000} \\
Asy & Stride & CT & IQR  &   \textbf{0.008} &            \textbf{0.008} &                   0.012 &  \textbf{0.008} &          0.011 \\
Asy & Stride & PD & bias &   \textbf{0.000} &            \textbf{0.000} &           \textbf{0.000} &         -0.006 &  \textbf{0.000} \\
Asy & Stride & PD & IQR  &           0.012 &                    0.012 &                   0.012 &          0.052 &  \textbf{0.008} \\
Asy & Stance & CT & bias &          -0.008 &                   -0.004 &                  -0.008 &  \textbf{0.000} &         -0.006 \\
Asy & Stance & CT & IQR  &           0.027 &                    0.016 &                   0.025 &  \textbf{0.012} &          0.020 \\
Asy & Stance & PD & bias &          -0.008 &                   -0.008 &                  -0.012 &  \textbf{0.000} &         -0.006 \\
Asy & Stance & PD & IQR  &           0.032 &                    0.027 &                   0.027 &  \textbf{0.016} &          0.025 \\
Asy & Swing & CT & bias  &          -0.008 &                   -0.004 &                  -0.006 &  \textbf{0.000} &         -0.004 \\
Asy & Swing & CT & IQR   &           0.023 &                    0.020 &                   0.016 &  \textbf{0.012} &          0.016 \\
Asy & Swing & PD & bias  &          -0.008 &                   -0.006 &                  -0.012 &  \textbf{0.000} &  \textbf{0.000} \\
Asy & Swing & PD & IQR   &           0.031 &            \textbf{0.020} &                   0.027 &          0.023 &          0.023 \\
\bottomrule
\end{tabular}

